The Arity Hierarchy in the Polyadic $\mu$-Calculus

The polyadic mu-calculus is a modal fixpoint logic whose formulas define relations of nodes rather than just sets in labelled transition systems. It can express exactly the polynomial-time computable and bisimulation-invariant queries on finite graphs. In this paper we show a hierarchy result with respect to expressive power inside the polyadic mu-calculus: for every level of fixpoint alternation, greater arity of relations gives rise to higher expressive power. The proof uses a diagonalisation argument.

==> eptcsdata.tex <==
\providecommand{\firstpage}{105}
\providecommand{\publicationstatus}{R. Matthes, M. Mio (Eds.): Fixed Points\\
in Computer Science 2015 (FICS 2015)\\
EPTCS 191, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.191.10}{10.4204/EPTCS.191.10}}
\pdfoutput=1

